PolicyGuard: From Organizational Policies to Neuro-SymbolicCompliance Review Engines

Policy-grounded document review requires determining whether a target document complies with organization-specific policies, guidelines, or playbooks. While large language models can assist with policy interpretation and document analysis, end-to-end prompting leaves the applied policy logic implicit, making compliance decisions difficult to inspect, update, and test. We present PolicyGuard, a neuro-symbolic framework for policy-grounded document compliance review. PolicyGuard converts organizational policy guidance into an executable review engine consisting of typed relational logic rules and atom-level extraction questions. During review, LLMs answer these local questions using retrieved document evidence, and a symbolic evaluator applies the formal rules to detect non-compliance. We instantiate and evaluate PolicyGuard on company-specific NDA compliance review, where contract clauses must be checked against organization-specific negotiation policies. By separating policy formalization, local document interpretation, and symbolic compliance evaluation, PolicyGuard makes document review more explicit, maintainable, and systematically testable.

==> paper/sections/method_v2.tex <==
\begin{figure*}[!t]
    \centering

    \includegraphics[width=0.88\textwidth]{figures/review_engine_builder.png}

    \vspace{0.4em}

    \includegraphics[width=0.88\textwidth]{figures/inference.png}

    \caption{Overview of the PolicyGuard pipeline. The upper figure shows the review-engine construction process, where policy guidance is converted into formal artifacts and validated through a repair loop. The lower figure shows the inference-time review process, where a target document is segmented, routed, converted into frames and facts, and evaluated against symbolic policy rules.}
    \label{fig:method-overview}
\end{figure*}


\section{PolicyGuard}
\label{sec:method}
\subsection{Overview}
\label{sec:policyguard-overview}

PolicyGuard is a neuro-symbolic framework for policy-grounded document review. Given a company policy, it builds a review engine that determines whether a target document violates that policy. We instantiate PolicyGuard for NDA review, where the goal is to detect contractual provisions that conflict with a company's negotiation policy.

PolicyGuard has two phases. In the build phase, policy rulecards are converted into formal logic specifications over a shared ontology, and a corresponding extraction layer is constructed to map contract text into the facts required by those rules. The build phase also enriches the ontology with legal evaluation semantics, constructs a reusable frame catalog with extraction guidance, groups related frames into extraction bundles, and validates the resulting engine through end-to-end rule tests.

In the inference phase, a target NDA is segmented into clauses, relevant extraction bundles are applied, extracted frames are expanded into ontology-level facts, and a symbolic evaluator executes the policy rules over the resulting document-level fact graph. Thus, LLMs are used to construct, repair, and locally extract structured legal content, while the final compliance decision is produced by deterministic symbolic inference.

\subsection{Building the Review Engine}
\label{sec:engine-builder}

\paragraph{Rulecard construction.}
PolicyGuard first converts the policy into self-contained policy units. Each policy unit is organized around a single contract review issue and contains the policy text and contextual material needed to interpret that issue. From each unit, PolicyGuard extracts a verifiable compliance-violation rule. The rule remains in natural language, but it explicitly states the condition, whether by the presence or absence of contractual language, under which the target document violates the policy. This separates the operative review criterion from surrounding explanations, preferences, examples, and drafting guidance. Metadata such as the company position, violation category, risk posed, target party, severity, and explanation is recorded alongside the rule.

\paragraph{Formalizing policies and ontology semantics.}
Each natural-language compliance-violation rule is translated into a finite typed relational logic specification that can be evaluated over a document-level fact graph. The fact graph represents legally relevant content extracted from a target document. Its nodes are typed legal objects, such as obligations, disclosures, purposes, parties, durations, or information categories, and its edges represent relations between those objects. In the logic specification, variables range over typed objects, unary predicates assign object types or properties, binary predicates express relations between objects, and constants denote canonical legal categories or thresholds. A rule fires when all atoms in its positive body are satisfied and no assignment satisfies its negative existential conditions, which represent blocking exceptions or required absences.

Formalization is performed against a shared global ontology of sorts, predicates, and constants. When a rule requires a concept that is not yet represented, the formalizer proposes new ontology vocabulary rather than introducing purely local symbols. Crucially, PolicyGuard also generates legal evaluation semantics for every new predicate and for constants whose interpretation affects rule evaluation. These semantics describe the legal meaning of the term, the textual conditions under which it should be treated as true, and the boundary between satisfying and non-satisfying language. They are generated at the point of rulecard formalization because the rulecard contains the policy context needed to state the intended meaning precisely.

The legal evaluation semantics make the ontology more than a list of symbol names. They allow later rulecards to understand and reuse existing vocabulary instead of creating redundant or slightly incompatible predicates. They also improve canonicality: two rulecards that express the same legal concept in different surface language are more likely to map to the same ontology term when that term carries an explicit semantic definition. This reduces ontology drift and produces a more stable symbolic layer for downstream extraction and evaluation.

\paragraph{Building the frame catalog.}
The logic specifications define which facts are needed to detect policy violations, but not how those facts should be obtained from contract text. PolicyGuard therefore constructs a frame catalog that serves as the text-to-logic interface. A frame type represents an extractable legal object, such as a confidentiality obligation, a permitted disclosure, a disclosure condition, a purpose definition, a receiving party, an information category, or a survival period. Each frame type specifies the attributes needed to expand that object into ontology-level facts. Attributes may contain canonical constants, references to other extracted frames, primitive values, or boolean assertions.

The frame catalog is generated from the logic specifications together with the ontology and its legal evaluation semantics. The semantics help determine which distinctions must be preserved for rule evaluation and which surface variations are merely drafting differences. As a result, frame types are not created mechanically from individual predicates. Instead, they are designed around reusable legal objects that can support many rules. This produces a smaller and more coherent catalog, avoids duplicative frame types, and improves the chance that future policy rules can be supported by the same extraction layer.

Each frame type includes frame-level extraction guidance explaining when that frame should be extracted from NDA text. Each attribute also includes attribute-level guidance explaining how to identify, normalize, and populate the field. For example, attribute guidance may explain how to recognize a prior-written-consent condition, how to distinguish a broad purpose clause from a transaction-specific purpose clause, or how to decide whether a designation right is prospective only or can cure prior disclosure retroactively. Because this guidance is grounded in the ontology's legal evaluation semantics, it is better aligned with the symbolic predicates that will later consume the extracted facts.

\paragraph{Constructing extraction bundles.}
After the frame catalog is built, PolicyGuard groups frame types into extraction bundles. A bundle contains frame types that are semantically related and are likely to be expressed in the same clauses or neighboring clauses. For example, frames concerning permitted disclosures, disclosure recipients, consent conditions, and safeguards may form one bundle, while purpose definitions and use restrictions may form another. Bundling gives the extractor enough local context to recover linked legal objects and object references, while keeping each extraction call focused on a coherent family of meanings.

\paragraph{End-to-end rule validation.}
Because the review engine is assembled from several generated components, a rule must be validated through the full inference pipeline rather than only by inspecting its formal specification. A rule may fail if the formalized condition is misaligned with the policy intent, if the frame guidance is underspecified, if linked legal objects are not extracted together, or if extracted frames are not expanded into the facts expected by the evaluator. PolicyGuard therefore validates each rulecard using rule-specific validation examples with known expected outcomes. For a violation example, a contract clause is constructed to instantiate the compliance-violation condition and is run through the same pipeline used during review, where the corresponding rule is expected to fire. In our NDA setting, we construct these examples by prompting an LLM to rewrite compliant clauses from the company template into non-compliant variants; the rewritten clauses are manually verified before use. If the observed outcome differs from the expected outcome, the failed run provides a trace of intermediate outputs, which is used to identify and repair the responsible generated artifact. Repairs are restricted to the logic specification and the frame catalog: logic-specification repairs correct misformalized rule conditions, while frame-catalog repairs may update extraction guidance, add missing attributes, refine canonical categories, or add object-reference fields linking related legal objects.

\subsection{Policy-Grounded Document Review}
\label{sec:inference-time-review}

At inference time, PolicyGuard applies the constructed review engine to a target contract by converting natural-language clauses into a finite fact graph and evaluating the policy rules over it. The contract is first segmented into clauses. Relevant extraction bundles are selected for each clause, and the corresponding extractors produce structured frames for the legal objects expressed in the text. These frames may include canonical attribute values, primitive values, and references to other frames when the clause expresses linked legal objects.

A deterministic fact expansion step maps the extracted frames into ontology-level facts: typed objects, properties, constants, and relations. The symbolic evaluator then executes each formal rule over the resulting document-level fact graph. Variables range over extracted objects of the appropriate sorts, positive atoms must be present in the graph, and negative existential conditions are evaluated under the closed-world assumption. When a rule body is satisfied, PolicyGuard emits the corresponding policy risk together with an evaluation trace showing the supporting bindings and facts. Thus, inference combines local LLM-based extraction with deterministic reasoning over the complete document.

% \section{PolicyGuard}
% \label{sec:method}

% \subsection{Overview}
% \label{sec:policyguard-overview}

% PolicyGuard is a neuro-symbolic framework for policy-grounded document review. Given a company policy, it builds a review engine that analyzes whether a target document complies with that policy. We instantiate PolicyGuard for NDA review, where the goal is to detect contractual provisions that conflict with a company's negotiation policy.

% PolicyGuard has two phases. In the build phase, policy rulecards are formalized into finite typed relational logic specifications over a shared ontology of canonical sorts, constants, and predicates. PolicyGuard also constructs an extraction layer that maps contract clauses into the structured facts required by these rules. The resulting engine is validated and repaired at two levels: deterministic static checks verify that the extraction layer can support the predicates, variables, and relational atoms required by the logic specifications, while synthetically risky NDA articles test whether each rule can actually fire through the end-to-end inference pipeline. Failures at either level trigger LLM-based repair of the relevant components.

% In the inference phase, a target NDA is segmented into clauses, routed to relevant extractors, converted into structured frames, and expanded into ontology-level facts. A symbolic evaluator then executes the logic rules over the document-level fact graph and emits policy risks when rule bodies are satisfied. Thus, LLMs are used to construct, repair, and locally extract structured legal content, while the final compliance decision is produced by deterministic symbolic inference.

% \subsection{Building the Review Engine}
% \label{sec:engine-builder}

% \paragraph{Rulecard construction.}
%  PolicyGuard first converts the policy into self-contained policy units, each organized around a single contract review issue and containing the policy text and contextual material needed to interpret that issue. From each policy unit, PolicyGuard extracts a verifiable compliance-violation rule. The rule is still expressed in natural language, but it explicitly states the condition, whether by presence or absence of contractual language, under which the target document violates the policy. This separates the operative review criterion from surrounding explanations, preferences, examples, and drafting guidance in the policy text. Metadata such as the company position, violation category, risk posed, target party, severity, and explanation is then recorded alongside the rule.

% \paragraph{Formalizing policies.}
% Each natural-language compliance-violation rule is translated into a finite typed relational logic specification that can be evaluated over a document-level fact graph. The fact graph represents the legally relevant content extracted from a target document. Its nodes are typed legal objects, such as obligations, disclosures, purposes, parties, durations, or information categories, and its edges represent relations between those objects. In the logic specification, variables range over these typed objects, unary predicates assign object types or properties, binary predicates express relations between objects, and constants denote canonical legal categories or thresholds. A rule fires when all atoms in its positive body are satisfied and no assignment satisfies its negative existential conditions, which are used to represent blocking exceptions or required absences.

% Formalization is performed against a shared global ontology of sorts, constants, and predicates. When a rule requires a concept that is not yet represented, the formalizer proposes new ontology vocabulary rather than introducing purely local symbols. These proposals are validated before being added to the ontology, allowing later rules to reuse previously introduced symbolic representations.

% \paragraph{Building the text-to-logic interface.}
% The logic specifications define the facts needed to detect a policy risk, but not how those facts are obtained from contract text. PolicyGuard therefore builds a text-to-logic interface from the logic specifications. This interface identifies the legal objects that must be extractable from NDA clauses, such as obligations, exceptions, durations, parties, information categories, disclosure conditions, or permitted-use restrictions. For each object type, it specifies the fields needed to express the object as rule predicates during fact expansion.

% The interface also specifies which kinds of clauses should be inspected for each kind of legal object. This focuses extraction on contract language that can produce facts required by the rules, while avoiding a full-document search for every possible legal pattern. PolicyGuard then performs deterministic support checks to verify that this interface can produce the predicates, variables, and relational atoms required by each rule body, including atoms in negative existential conditions. Unsupported predicates, missing variable support, incompatible sorts, or infeasible relations trigger LLM-based repair followed by rechecking.

% \paragraph{End-to-end rule validation.}
% The support checks above verify that the text-to-logic interface can, in principle, supply the facts required by the rules. However, a rule may still fail end-to-end if the formalized condition is misaligned with the policy intent, if relevant clauses are inspected incorrectly, or if extracted structures are not expanded into the facts expected by the evaluator. PolicyGuard therefore validates each rulecard separately using a rule-specific validation example. For each rulecard, a contract clause is constructed to instantiate the extracted violation condition and is run through the same inference pipeline used during review, where the corresponding rule is expected to fire. In our NDA setting, we construct these examples by prompting an LLM to rewrite compliant clauses from the company template into non-compliant variants; the rewritten clauses are manually verified before use. If the expected rule does not fire, the failed run provides a trace of intermediate outputs, which is used to identify and repair the responsible part of the constructed engine.

% \subsection{Policy-Grounded Document Review}
% \label{sec:inference-time-review}

% At inference time, PolicyGuard applies the constructed review engine to a target contract by converting natural-language clauses into a finite fact graph and evaluating the policy rules over it. The contract is first segmented into clauses. Using the text-to-logic interface built earlier, each clause is inspected for the legal objects relevant to the policy rules, such as obligations, exceptions, information categories, conditions, and time limits. The result is a set of structured representations of clause meaning.

% A deterministic fact expansion step maps these structured representations into ontology-level facts: typed objects, properties, and relations. The symbolic evaluator then executes each formal rule over the resulting document-level fact graph. Variables range over extracted objects of the appropriate sorts, positive atoms must be present in the graph, and negative existential conditions are evaluated under the closed-world assumption. When a rule body is satisfied, PolicyGuard emits the corresponding policy risk together with an evaluation trace showing the supporting bindings and facts. Thus, inference combines local LLM-based extraction with deterministic reasoning over the complete document.
